Definition-Guided In-Context Learning for Zero-Shot Spoken Language Understanding

Adapting spoken language understanding (SLU) systems to novel or revised label taxonomies conventionally requires additional labeled data and retraining, creating a bottleneck for real world deployment. While in-context learning with few-shot demonstrations offers an alternative, multi-modal generalization and scaling has been challenging. In this work, we investigate whether natural-language definitions alone can guide zero-shot SLU without demonstration exemplars, finding that symbolic definitions serve as the primary supervisory driver for adapting speech-text models. We operationalize this principle as Definition-Guided In-Context Learning (DG-ICL), a fine-tuning framework that decouples semantic categories from fixed lexical names. By replacing labels with dynamically randomized definitions (arbitrary synthetic tokens in DG-ICL-Sym or permuted vocabulary words in DG-ICL-Flip), DG-ICL avoids lexical shortcuts and encourages the model to ground acoustic representations in contextual definitions. Novel categories can thus be introduced at inference simply by defining them through the instructions. Across three speech-text models (AUDIO FLAMINGO 3, QWEN2-AUDIO, and SALMONN), DG-ICL outperforms standard instruction tuning on held-out tasks under novel symbols (0.663 vs. 0.449 macro-F1 on Audio Flamingo 3; 0.703 vs. 0.620 on Qwen2-Audio; 0.582 vs. 0.399 on SALMONN), while remaining competitive on original labels. Furthermore, counterfactual evaluations demonstrate instruction following abilities, where it is shown that DG-ICL-Sym retains 68% of its performance when definitions contradict pre-trained lexical priors, whereas standard instruction tuning elicits significantly reduced retention of 21%. Finally, we show that DG-ICL enables zero-shot speech clustering into user-defined categories specified on the fly

==> tables/definitions_vs_demonstrations.tex <==
\begin{table}[t]
\centering
\small
\caption{Held-out zero-shot versus few-shot performance (macro-F1) across prompt information regimes on \textsc{Audio Flamingo~3}. Each model is evaluated under three prompt conditions: label definitions only ($k=0$), one demonstration per class only ($k=1$), or both combined. Definitions alone drive the highest performance in \methodsym{}, surpassing all baseline configurations regardless of exemplar availability. Values report mean\,{\scriptsize($\pm$std)} over three seeds; best overall average in \textbf{bold}.}
\label{tab:def-vs-demo}
\begin{tabular}{lccc}
\toprule
Method & Definitions & Demonstrations & Both \\
\midrule
Instruction Tuning                  & 0.449\,{\scriptsize($\pm$.041)} & 0.239\,{\scriptsize($\pm$.040)} & 0.480\,{\scriptsize($\pm$.025)} \\
Symbol Tuning~\cite{wei2023symbol}  & 0.460\,{\scriptsize($\pm$.018)} & 0.484\,{\scriptsize($\pm$.010)} & 0.445\,{\scriptsize($\pm$.055)} \\
\methodsym{} (ours)                 & \textbf{0.663}\,{\scriptsize($\pm$.021)} & 0.336\,{\scriptsize($\pm$.038)} & 0.640\,{\scriptsize($\pm$.033)} \\
\methodflip{} (ours)                & 0.534\,{\scriptsize($\pm$.029)} & 0.248\,{\scriptsize($\pm$.052)} & 0.513\,{\scriptsize($\pm$.031)} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/dynamic_vs_static.tex <==
\begin{table}[t]
\centering\small
\caption{Dynamic versus static symbol assignment (macro-F1 on \textsc{Audio Flamingo~3}). Static symbol tuning binds categories to an invariant bijective mapping throughout training, whereas \methodsym{} samples dynamic bijections per training instance. Dynamic re-randomization is the key mechanism enabling the model to generalize zero-shot to novel symbolic taxonomies on held-out tasks. Values report mean\,{\scriptsize($\pm$std)} (Static $n{=}2$, \methodsym{} $n{=}3$); best held-out symbolic performance in \textbf{bold}.}
\label{tab:dynamic-vs-static}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Original labels} & \multicolumn{2}{c}{Symbolic labels} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Method & Trained & Held-out & Trained & Held-out \\
\midrule
Static (fixed map) & 0.679\,{\scriptsize($\pm$.004)} & 0.746\,{\scriptsize($\pm$.002)} & 0.515\,{\scriptsize($\pm$.071)} & 0.426\,{\scriptsize($\pm$.012)} \\
\methodsym{} (ours)   & 0.762\,{\scriptsize($\pm$.005)} & 0.766\,{\scriptsize($\pm$.026)} & 0.638\,{\scriptsize($\pm$.045)} & \textbf{0.663}\,{\scriptsize($\pm$.021)} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/flipped_demonstration_sweep.tex <==
\begin{table}[t]
\centering
\caption{Effect of adding few-shot demonstrations to our flipped-label model (\methodflip{}) at inference. Across total demonstration budgets $m \in \{0, 1, 5, 10\}$, demonstrations yield no consistent improvement over the zero-shot baseline ($m=0$), and fail to close the gap to \methodsym{}'s zero-shot performance ($0.663$). Values report mean\,{\scriptsize($\pm$std)} over three seeds.}
\label{tab:agrawal}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Held-out} & \multicolumn{2}{c}{Trained} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
$m$ & Original & Symbolic & Original & Symbolic \\
\midrule
0  & 0.780\,{\scriptsize($\pm$.005)} & 0.534\,{\scriptsize($\pm$.029)} & 0.817\,{\scriptsize($\pm$.004)} & 0.546\,{\scriptsize($\pm$.053)} \\
\midrule
1  & 0.752\,{\scriptsize($\pm$.004)} & 0.485\,{\scriptsize($\pm$.070)} & 0.810\,{\scriptsize($\pm$.004)} & 0.558\,{\scriptsize($\pm$.066)} \\
5  & 0.759\,{\scriptsize($\pm$.008)} & 0.547\,{\scriptsize($\pm$.072)} & 0.805\,{\scriptsize($\pm$.006)} & 0.588\,{\scriptsize($\pm$.023)} \\
10 & 0.757\,{\scriptsize($\pm$.009)} & 0.513\,{\scriptsize($\pm$.034)} & 0.801\,{\scriptsize($\pm$.003)} & 0.462\,{\scriptsize($\pm$.036)} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/it_demonstration_sweep.tex <==
\begin{table}[t]
\centering
\caption{Demonstration scaling sweep on Instruction Tuning (symbolic-label macro-F1 across held-out and fine-tuning tasks). As demonstrations per class ($k$) increase, performance plateaus and fails to approach the zero-shot generalization of \methodsym{}. Values report mean\,{\scriptsize($\pm$std)} over three seeds; best overall in \textbf{bold}.}
\label{tab:ksweep}
\begin{tabular}{lcc}
\toprule
Setting & Held-out & Trained \\
\midrule
Instruction Tuning, $k{=}0$ (zero-shot) & 0.449\,{\scriptsize($\pm$.041)} & 0.508\,{\scriptsize($\pm$.028)} \\
Instruction Tuning, $k{=}1$              & 0.480\,{\scriptsize($\pm$.025)} & 0.518\,{\scriptsize($\pm$.050)} \\
Instruction Tuning, $k{=}2$              & 0.504\,{\scriptsize($\pm$.026)} & 0.478\,{\scriptsize($\pm$.015)} \\
Instruction Tuning, $k{=}3$              & 0.499\,{\scriptsize($\pm$.046)} & 0.429\,{\scriptsize($\pm$.021)} \\
\midrule
\methodsym{} (ours), zero-shot              & \textbf{0.663}\,{\scriptsize($\pm$.021)} & \textbf{0.638}\,{\scriptsize($\pm$.044)} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/multitask_breadth.tex <==
\begin{table}[t]
\centering
\caption{Effect of multi-task training breadth on held-out symbolic macro-F1 (test split). Increasing fine-tuning task diversity improves out-of-distribution transfer across methods, with \methodsym{} outperforming standard Instruction Tuning across all task counts. Values report mean\,{\scriptsize($\pm$std)} over three seeds; best per-column performance in \textbf{bold}.}
\label{tab:breadth}
\begin{tabular}{lccc}
\toprule
Method & 1-task & 2-task & 3-task \\
\midrule
Pre-trained          & 0.320 & 0.320 & 0.320 \\
Instruction Tuning & 0.369\,{\scriptsize($\pm$.030)} & 0.341\,{\scriptsize($\pm$.009)} & 0.449\,{\scriptsize($\pm$.041)} \\
\methodsym{} (ours)   & \textbf{0.532}\,{\scriptsize($\pm$.017)} & \textbf{0.524}\,{\scriptsize($\pm$.035)} & \textbf{0.663}\,{\scriptsize($\pm$.021)} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/speech_clustering.tex <==
\begin{table}[t]
\centering
\small
\caption{Zero-shot speech clustering performance into user-defined categories (test split), averaged over Skit-S2I and MInDS-14 (French and Korean). Each category is specified by an invariant natural-language definition across three controlled naming styles (Meaningful, Neutral, Symbolic). Under meaningful and neutral names, all models perform comparably; under symbolic names, standard Instruction Tuning and the pre-trained foundation model collapse, while the decoupling family (\methodsym{}, \methodflip{}, and Symbol Tuning) retains invariant accuracy across both audio and text modalities. Values report mean\,{\scriptsize($\pm$std)} over three seeds; best symbolic performance in \textbf{bold}.}
\label{tab:cluster}
\begin{tabular}{llccccc}
\toprule
Query & Style & \methodsym{} & \methodflip{} & Symbol Tun. & Instr. Tun. & Pre-trained \\
\midrule
\multirow{3}{*}{Audio}
 & Meaningful & 0.679\,{\scriptsize($\pm$.016)} & 0.697\,{\scriptsize($\pm$.009)} & 0.659\,{\scriptsize($\pm$.010)} & 0.636\,{\scriptsize($\pm$.007)} & 0.608 \\
 & Neutral    & 0.671\,{\scriptsize($\pm$.008)} & 0.698\,{\scriptsize($\pm$.011)} & 0.678\,{\scriptsize($\pm$.011)} & 0.643\,{\scriptsize($\pm$.007)} & 0.661 \\
 & Symbolic   & 0.679\,{\scriptsize($\pm$.005)} & \textbf{0.696}\,{\scriptsize($\pm$.008)} & 0.662\,{\scriptsize($\pm$.006)} & 0.396\,{\scriptsize($\pm$.007)} & 0.379 \\
\midrule
\multirow{3}{*}{Text}
 & Meaningful & 0.727\,{\scriptsize($\pm$.011)} & 0.748\,{\scriptsize($\pm$.016)} & 0.717\,{\scriptsize($\pm$.011)} & 0.695\,{\scriptsize($\pm$.006)} & 0.703 \\
 & Neutral    & 0.758\,{\scriptsize($\pm$.008)} & 0.750\,{\scriptsize($\pm$.007)} & 0.735\,{\scriptsize($\pm$.010)} & 0.731\,{\scriptsize($\pm$.008)} & 0.734 \\
 & Symbolic   & 0.747\,{\scriptsize($\pm$.005)} & \textbf{0.752}\,{\scriptsize($\pm$.009)} & 0.733\,{\scriptsize($\pm$.015)} & 0.469\,{\scriptsize($\pm$.019)} & 0.435 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/steerability_counterfactual.tex <==

\begin{table}[t]
\centering\small
\caption{Instruction steerability under counterfactual definition mappings on held-out tasks (macro-F1). Held-out performance is reported before (Original) and after (Counterfactual) label-definition derangement, alongside the retention percentage ($\text{Retained} = \text{Counterfactual} / \text{Original}$). While standard baselines collapse to 17\% to 21\% by reverting to pre-trained lexical priors, \methodsym{} retains 68\% of its performance by actively tracking the definition text, with \methodflip{} providing a matched-derangement ceiling. Values report mean\,{\scriptsize($\pm$std)} over three seeds; best non-ceiling results in \textbf{bold}.}
\label{tab:flip}
\begin{tabular}{lccc}
\toprule
Method & Original & Counterfactual & Retained \\
\midrule
Pre-trained                          & 0.630 & 0.105 & 17\% \\
Instruction Tuning                  & 0.772\,{\scriptsize($\pm$.002)} & 0.165\,{\scriptsize($\pm$.026)} & 21\% \\
Symbol Tuning~\cite{wei2023symbol}  & 0.692\,{\scriptsize($\pm$.016)} & 0.326\,{\scriptsize($\pm$.054)} & 47\% \\
\methodsym{} (ours)                 & 0.766\,{\scriptsize($\pm$.026)} & \textbf{0.522}\,{\scriptsize($\pm$.057)} & \textbf{68\%} \\
\midrule
\multicolumn{4}{l}{\textit{Matched-training ceiling (trained on derangements):}} \\
\methodflip{} (ours)                & 0.780\,{\scriptsize($\pm$.004)} & 0.784\,{\scriptsize($\pm$.016)} & ${\sim}100\%$ \\
\bottomrule
\end{tabular}
\end{table}


